Shifts: A Dataset of Real Distributional Shift Across Multiple Large-Scale Tasks

There has been significant research done on developing methods for improving robustness to distributional shift and uncertainty estimation. In contrast, only limited work has examined developing standard datasets and benchmarks for assessing these approaches. Additionally, most work on uncertainty estimation and robustness has developed new techniques based on small-scale regression or image classification tasks. However, many tasks of practical interest have different modalities, such as tabular data, audio, text, or sensor data, which offer significant challenges involving regression and discrete or continuous structured prediction. Thus, given the current state of the field, a standardized large-scale dataset of tasks across a range of modalities affected by distributional shifts is necessary. This will enable researchers to meaningfully evaluate the plethora of recently developed uncertainty quantification methods, as well as assessment criteria and state-of-the-art baselines. In this work, we propose the Shifts Dataset for evaluation of uncertainty estimates and robustness to distributional shift. The dataset, which has been collected from industrial sources and services, is composed of three tasks, with each corresponding to a particular data modality: tabular weather prediction, machine translation, and self-driving car (SDC) vehicle motion prediction. All of these data modalities and tasks are affected by real, "in-the-wild" distributional shifts and pose interesting challenges with respect to uncertainty estimation. In this work we provide a description of the dataset and baseline results for all tasks.

==> poster/abbreviations.tex <==
% Abbreviations

\newcommand{\iid}{independent and identically distributed\xspace}

\newcommand{\logl}{log-likelihood\xspace}
\newcommand{\Logl}{Log-likelihood\xspace}
\newcommand{\LL}{\textsc{ll}\xspace}
\newcommand{\logls}{{\logl}s\xspace}
\newcommand{\Logls}{{\Logl}s\xspace}
\newcommand{\LLs}{{\LL}s\xspace}

\newcommand{\mlh}{maximum likelihood\xspace}
\newcommand{\Mlh}{Maximum likelihood\xspace}
\newcommand{\ML}{\textsc{ml}\xspace}

\newcommand{\mle}{maximum-likelihood estimation\xspace}
\newcommand{\Mle}{Maximum-likelihood estimation\xspace}
\newcommand{\MLE}{\textsc{mle}\xspace}
\newcommand{\mlee}{maximum-likelihood estimate\xspace}
\newcommand{\mled}{maximum-likelihood estimated\xspace}
\newcommand{\mles}{maximum-likelihood estimates\xspace}

\newcommand{\map}{maximum \emph{a posteriori}\xspace}
\newcommand{\Map}{Maximum \emph{a posteriori}\xspace}
\newcommand{\MAP}{\textsc{map}\xspace}

\newcommand{\cml}{conditional maximum likelihood\xspace}
\newcommand{\Cml}{Conditional maximum likelihood\xspace}
\newcommand{\CML}{\textsc{cml}\xspace}

\newcommand{\mbr}{minimum Bayes risk\xspace}
\newcommand{\Mbr}{Minimum Bayes risk\xspace}
\newcommand{\MBR}{\textsc{mbr}\xspace}

\newcommand{\mpe}{minimum phone error\xspace}
\newcommand{\Mpe}{Minimum phone error\xspace}
\newcommand{\MPE}{\textsc{mpe}\xspace}

\newcommand{\expm}{expect\-ation--maxi\-misation\xspace}
\newcommand{\Expm}{Expect\-ation--maxi\-misation\xspace}
\newcommand{\EM}{\textsc{em}\xspace}

\newcommand{\kl}{Kullback-Leibler\xspace}
\newcommand{\Kl}{\kl}
\newcommand{\KL}{\textsc{kl}\xspace}

% Techniques

\newcommand{\mllr}{maximum-likelihood linear regression\xspace}
\newcommand{\Mllr}{Maximum-likelihood linear regression\xspace}
\newcommand{\MLLR}{\textsc{mllr}\xspace}
\hyphenation{mllr}

\newcommand{\fe}{front-end}
\newcommand{\Fe}{Front-end}
\newcommand{\FE}{\textsc{fe}}

\newcommand{\cmllr}{constrained \mllr}
\newcommand{\Cmllr}{Constrained \mllr}
\newcommand{\CMLLR}{\textsc{cmllr}\xspace}
\hyphenation{cmllr}

\newcommand{\lda}{linear discriminant analysis\xspace}
\newcommand{\Lda}{Linear discriminant analysis\xspace}
\newcommand{\LDA}{\textsc{lda}\xspace}

\newcommand{\hda}{heteroscedastic discriminant analysis\xspace}
\newcommand{\Hda}{Heteroscedastic discriminant analysis\xspace}
\newcommand{\HDA}{\textsc{hda}\xspace}

\newcommand{\hlda}{heteroscedastic \lda{}\xspace}
\newcommand{\Hlda}{Heteroscedastic \lda{}\xspace}
\newcommand{\HLDA}{\textsc{hlda}\xspace}
\hyphenation{hlda}

\newcommand{\mhlda}{multiple \hlda{}\xspace}
\newcommand{\Mhlda}{Multiple \hlda{}\xspace}
\newcommand{\MHLDA}{\textsc{mhlda}\xspace}
\hyphenation{mhlda}

\newcommand{\mlda}{multiple \lda{}\xspace}
\newcommand{\Mlda}{Multiple \lda{}\xspace}
\newcommand{\MLDA}{\textsc{mlda}\xspace}
\hyphenation{mlda}

\newcommand{\VTLN}{\textsc{vtln}\xspace}
\newcommand{\Vtln}{Vocal tract length normalisation\xspace}
\newcommand{\vtln}{vocal tract length normalisation\xspace}

% Noise-robustness techniques and such

\newcommand{\dft}{discrete Fourier transform\xspace}
\newcommand{\Dft}{Discrete Fourier transform\xspace}
\newcommand{\DFT}{\textsc{dft}\xspace}

\newcommand{\dct}{discrete cosine transform\xspace}
\newcommand{\Dct}{Discrete cosine transform\xspace}
\newcommand{\DCT}{\textsc{dct}\xspace}

\newcommand{\mfcc}{Mel-frequency cepstral coefficient\xspace}
\newcommand{\Mfcc}{\mfcc}
\newcommand{\MFCC}{\textsc{mfcc}\xspace}
\newcommand{\mfccs}{{\mfcc}s\xspace}
\newcommand{\Mfccs}{{\Mfcc}s\xspace}
\newcommand{\MFCCs}{{\MFCC}s\xspace}
\hyphenation{mfcc}
\hyphenation{mfccs}

\newcommand{\hmm}{hidden Markov model\xspace}
\newcommand{\Hmm}{Hidden Markov model\xspace}
\newcommand{\HMM}{\textsc{hmm}\xspace}
\newcommand{\hmms}{{\hmm}s\xspace}
\newcommand{\Hmms}{{\Hmm}s\xspace}
\newcommand{\HMMs}{{\HMM}s\xspace}
\hyphenation{hmm}
\hyphenation{hmms}

\newcommand{\gmm}{Gaussian mixture model\xspace}
\newcommand{\Gmm}{\gmm}
\newcommand{\GMM}{\textsc{gmm}\xspace}
\newcommand{\gmms}{{\gmm}s\xspace}
\newcommand{\Gmms}{{\Gmm}s\xspace}
\newcommand{\GMMs}{{\GMM}s\xspace}
\hyphenation{gmm}
\hyphenation{gmms}

\newcommand{\igmm}{infinite \gmm}
\newcommand{\iGMM}{infinite \GMM}
\newcommand{\Igmm}{Infinite \gmm}
\newcommand{\IGMM}{\textsc{igmm}\xspace}
\newcommand{\igmms}{{\igmm}s\xspace}
\newcommand{\iGMMs}{{\iGMM}s\xspace}
\newcommand{\Igmms}{{\Igmm}s\xspace}
\newcommand{\IGMMs}{{\IGMM}s\xspace}
\hyphenation{igmm}
\hyphenation{igmms}

\newcommand{\ihmm}{infinite \hmm}
\newcommand{\iHMM}{infinite \HMM}
\newcommand{\Ihmm}{Infinite \hmm}
\newcommand{\IHMM}{\textsc{ihmm}\xspace}
\newcommand{\ihmms}{{\ihmm}s\xspace}
\newcommand{\iHMMs}{{\iHMM}s\xspace}
\newcommand{\Ihmms}{{\Ihmm}s\xspace}
\newcommand{\IHMMs}{{\IHMM}s\xspace}

\newcommand{\mog}{mixture of Gaussians\xspace}
\newcommand{\Mog}{Mixture of Gaussians\xspace}
\newcommand{\MOG}{\textsc{m}o\textsc{g}\xspace}
\newcommand{\mogs}{mixtures of Gaussians\xspace}
\newcommand{\Mogs}{Mixtures of Gaussians\xspace}
\newcommand{\MOGs}{{\MOG}s\xspace}
\hyphenation{mog}
\hyphenation{mogs}

\newcommand{\fst}{finite-state transducer\xspace}
\newcommand{\Fst}{Finite-state transducer\xspace}
\newcommand{\FST}{\textsc{fst}\xspace}
\newcommand{\fsts}{{\fst}s\xspace}
\newcommand{\Fsts}{{\Fst}s\xspace}
\newcommand{\FSTs}{{\FST}s\xspace}

\newcommand{\fsa}{finite-state automaton\xspace}
\newcommand{\Fsa}{Finite-state automaton\xspace}
\newcommand{\FSA}{\textsc{fsa}\xspace}
\newcommand{\fsas}{finite-state automata\xspace}
\newcommand{\Fsas}{Finite-state automata\xspace}
\newcommand{\FSAs}{{\FSA}s\xspace}

\newcommand{\wfst}{weighted {\fst}\xspace}
\newcommand{\Wfst}{Weighted {\fst}\xspace}
\newcommand{\WFST}{\textsc{wfst}\xspace}
\newcommand{\wfsts}{{\wfst}s\xspace}
\newcommand{\Wfsts}{{\Wfst}s\xspace}
\newcommand{\WFSTs}{{\WFST}s\xspace}

\newcommand{\wfsa}{weighted {\fsa}\xspace}
\newcommand{\Wfsa}{Weighted {\fsa}\xspace}
\newcommand{\WFSA}{\textsc{wfsa}\xspace}
\newcommand{\wfsas}{weighted {\fsas}\xspace}
\newcommand{\Wfsas}{Weighted {\fsas}\xspace}
\newcommand{\WFSAs}{{\WFSA}s\xspace}

\newcommand{\crf}{conditional random field\xspace}
\newcommand{\Crf}{Conditional random field\xspace}
\newcommand{\CRF}{\textsc{crf}\xspace}
\newcommand{\crfs}{conditional random fields\xspace}
\newcommand{\Crfs}{Conditional random fields\xspace}
\newcommand{\CRFs}{\textsc{crf}s\xspace}

\newcommand{\svm}{support vector machine\xspace}
\newcommand{\Svm}{Support vector machine\xspace}
\newcommand{\SVM}{\textsc{svm}\xspace}
\newcommand{\svms}{{\svm}s\xspace}
\newcommand{\Svms}{{\Svm}s\xspace}
\newcommand{\SVMs}{{\SVM}s\xspace}

\newcommand{\ssvm}{structured {\svm}\xspace}
\newcommand{\sSVM}{structured {\SVM}\xspace}
\newcommand{\Ssvm}{Structured {\svm}\xspace}
\newcommand{\SSVM}{\textsc{ssvm}\xspace}
\newcommand{\ssvms}{{\ssvm}s\xspace}
\newcommand{\sSVMs}{{\sSVM}s\xspace}
\newcommand{\Ssvms}{{\Ssvm}s\xspace}
\newcommand{\SSVMs}{{\SSVM}s\xspace}

\newcommand{\spr}{single-pass retraining\xspace}
\newcommand{\Spr}{Single-pass retraining\xspace}
\newcommand{\SPR}{\textsc{spr}\xspace}
\newcommand{\spred}{single-pass retrained\xspace}
\newcommand{\Spred}{Single-pass retrained\xspace}


\newcommand{\mmse}{minimum mean square error\xspace}
\newcommand{\Mmse}{Minimum mean square error\xspace}
\newcommand{\MMSE}{\textsc{mmse}\xspace}
\hyphenation{mmse}

\newcommand{\mbfe}{model-based feature enhancement\xspace}
\newcommand{\Mbfe}{Model-based feature enhancement\xspace}
\newcommand{\MBFE}{\textsc{mbfe}\xspace}

\newcommand{\SPLICE}{\textsc{splice}\xspace}

\newcommand{\vts}{vector Taylor series\xspace}
\newcommand{\Vts}{Vector Taylor series\xspace}
\newcommand{\VTS}{\textsc{vts}\xspace}

\newcommand{\vat}{\VTS adaptive training\xspace}
\newcommand{\Vat}{\vat}
\newcommand{\VAT}{\textsc{vat}\xspace}

\newcommand{\dvat}{discriminative \VTS adaptive training\xspace}
\newcommand{\Dvat}{Discriminative \VTS adaptive training\xspace}
\newcommand{\DVAT}{\textsc{dvat}\xspace}

\newcommand{\cta}{continuous time approximation\xspace}
\newcommand{\Cta}{Continuous time approximation\xspace}
\newcommand{\CTA}{\textsc{cta}\xspace}
\hyphenation{cta}

\newcommand{\jud}{joint uncertainty decoding\xspace}
\newcommand{\Jud}{Joint uncertainty decoding\xspace}
\newcommand{\JUD}{\textsc{jud}\xspace}

\newcommand{\pmc}{parallel model combination\xspace}
\newcommand{\Pmc}{Parallel model combination\xspace}
\newcommand{\PMC}{\textsc{pmc}\xspace}

\newcommand{\dpmc}{data-driven parallel model combination\xspace}
\newcommand{\Dpmc}{Data-driven parallel model combination\xspace}
\newcommand{\DPMC}{\textsc{dpmc}\xspace}
\hyphenation{dpmc}

\newcommand{\idpmc}{iterative data-driven parallel model combination\xspace}
\newcommand{\Idpmc}{Iterative data-driven parallel model combination\xspace}
\newcommand{\IDPMC}{\textsc{idpmc}\xspace}
\hyphenation{idpmc}

\newcommand{\ut}{unscented transformation\xspace}
\newcommand{\Ut}{Unscented transformation\xspace}
\newcommand{\UT}{\textsc{ut}\xspace}

\newcommand{\stcm}{semi-tied covariance matrices\xspace}
\newcommand{\Stcm}{Semi-tied covariance matrices\xspace}
\newcommand{\pstcm}{predictive semi-tied covariance matrices\xspace}
\newcommand{\Pstcm}{Predictive semi-tied covariance matrices\xspace}

\newcommand{\pst}{predictive semi-tied\xspace}
\newcommand{\Pst}{Predictive semi-tied\xspace}
\newcommand{\PST}{\textsc{pst}\xspace}

\newcommand{\pcmllr}{predictive \cmllr}
\newcommand{\Pcmllr}{Predictive \cmllr}
\newcommand{\PCMLLR}{\textsc{pcmllr}\xspace}

\newcommand{\ncmllr}{noisy \cmllr}
\newcommand{\Ncmllr}{Noisy \cmllr}
\newcommand{\NCMLLR}{\textsc{ncmllr}\xspace}
\hyphenation{ncmllr}

\newcommand{\pncmllr}{predictive \ncmllr}
\newcommand{\Pncmllr}{Predictive \ncmllr}
\newcommand{\PNCMLLR}{\textsc{pncmllr}\xspace}
\hyphenation{pncmllr}


% Tools

\newcommand{\wer}{word error rate\xspace}
\newcommand{\Wer}{Word error rate\xspace}
\newcommand{\WER}{\textsc{wer}\xspace}
\newcommand{\wers}{{\wer}s\xspace}
\newcommand{\Wers}{{\Wer}s\xspace}
\newcommand{\WERs}{{\WER}s\xspace}

\newcommand{\ser}{sentence error rate\xspace}
\newcommand{\Ser}{Sentence error rate\xspace}
\newcommand{\SER}{\textsc{ser}\xspace}
\newcommand{\sers}{{\ser}s\xspace}
\newcommand{\Sers}{{\Ser}s\xspace}
\newcommand{\SERs}{{\SER}s\xspace}

\newcommand{\snr}{signal-to-noise ratio\xspace}
\newcommand{\Snr}{Signal-to-noise ratio\xspace}
\newcommand{\SNR}{\textsc{snr}\xspace}
\newcommand{\snrs}{{\snr}s\xspace}
\newcommand{\Snrs}{{\Snr}s\xspace}
\newcommand{\SNRs}{{\SNR}s\xspace}


\newcommand{\htk}{Hidden Markov Model Toolkit\xspace}
\newcommand{\Htk}{Hidden Markov Model Toolkit\xspace}
\newcommand{\HTK}{\textsc{htk}\xspace}

\newcommand{\SCARF}{\textsc{scarf}\xspace}
\newcommand{\ETSI}{\textsc{etsi}\xspace}

% Databases
%\newcommand{\rm}{Resource Management\xspace}
%\newcommand{\Rm}{\rm}
\newcommand{\RM}{\textsc{rm}\xspace}

\newcommand{\AURORA}{\textsc{aurora}\xspace}

\newcommand{\NOISEX}{\textsc{noisex}\xspace}

\newcommand{\TIDIGITS}{\textsc{tidigits}\xspace}

\newcommand{\DARPA}{\textsc{darpa}\xspace}

\newcommand{\NIST}{\textsc{nist}\xspace}

% Projects

\newcommand{\RREAP}{\textsc{r\textsuperscript{2}eap}\xspace}

% Conferences
\newcommand{\IEEE}{\textsc{ieee}\xspace}
\newcommand{\ICASSP}{\textsc{icassp}\xspace}



==> poster/math_notation.tex <==
\usepackage{keyval}
\usepackage{ifthen}
\usepackage{twoopt}

% Notation

\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\DefinedAs}{\triangleq}
\newcommand{\SetTo}{:=}
\newcommand{\ApproximatedAs}{\simeq}

\newcommand{\ExpectationSymbol}{\mathcal{E}}

% Spaces
\newcommand{\qqquad}{\qquad\qquad}
\newcommand{\qqqquad}{\qqquad\qqquad}

% General notation
\newcommand{\Parentheses}[2][]{\Delimiters[#1]{(}{#2}{)}}
\newcommand{\SquareBrackets}[2][]{\Delimiters[#1]{[}{#2}{]}}
\newcommand{\CurlyBrackets}[2][]{\Delimiters[#1]{\{}{#2}{\}}}
\newcommand{\AngleBrackets}[2][]{\Delimiters[#1]{\langle}{#2}{\rangle}}

\newcommand{\MidBar}[3][]{\Separator[#1]{#2}{|}{#3}}
\newcommand{\MidDoubleBar}[3][]{\Separator[#1]{#2}{\|}{#3}}
\newcommand{\MidBarP}[3][]{\Parentheses[#1]{\MidBar[#1]{#2}{#3}}}

\newcommand{\Given}[3][]{\MidBar[#1]{#2}{#3}}
\newcommand{\GivenP}[3][]{\MidBarP[#1]{#2}{#3}}

\newcommand{\Tuple}[2][]{\Parentheses[#1]{#2}}

% Operations
\newcommand{\Convolution}{*}
\newcommand{\Absolute}[2][]{\Delimiters[#1]{\lvert}{#2}{\rvert}}
\newcommand{\Determinant}[2][]{\Absolute[#1]{#2}}
\newcommand{\Norm}[2][]{\Delimiters[#1]{\|}{#2}{\|}}
\newcommand{\InnerProduct}[2]{\left\langle {#1},{#2} \right\rangle}
\newcommand{\Derivative}[2]{\frac{d #1 }{d #2}}
\newcommand{\DerivativeAt}[4]{\left.\frac{d #1 }{d #2 } #3 \right\rvert_{#4}}
\newcommand{\Partial}[2]{\frac{\partial #1 }{\partial #2}}
\newcommand{\PartialAt}[4]{\left.\frac{\partial #1 }{\partial #2 } #3 \right\rvert_{#4}}
\newcommand{\Integral}[2]{\int{#2} d{#1}}
\newcommand{\IntegralFromTo}[4]{\int_{#2}^{#3} {#4} d{#1}}
\newcommand{\OrderUnder}[2][]{O\Parentheses[#1]{#2}}
\newcommand{\OrderExact}[2][]{\Theta \Parentheses[#1]{#2}}
\newcommand{\OrderOver}[2][]{\Omega\Parentheses[#1]{#2}}

% Functions
\newcommand{\Exp}[1]{e^{#1}}
\newcommand{\ElementLog}{\mbox{\textbf{log}}}
\newcommand{\ElementExp}{\mbox{\textbf{exp}}}

\newcommand{\LogP}[2][]{\log\Parentheses[#1]{#2}}
\newcommand{\ElementLogP}[2][]{\ElementLog\Parentheses[#1]{#2}}

\newcommand{\ExpP}[2][]{\exp\Parentheses[#1]{#2}}
\newcommand{\ElementExpP}[2][]{\ElementExp\Parentheses[#1]{#2}}

\newcommand{\ElementTimes}{\circ}

\newcommand{\DeltaFunction}[3][]{\delta \Parentheses[#1]{ #2 = #3 }}
\newcommand{\KLDivergence}[3][]{\mathcal{KL} \Parentheses[#1]{\MidDoubleBar[#1]{#2}{#3}} }
\newcommand{\Entropy}[2][]{\mathcal{H} \Parentheses[#1]{ #2 } }
\newcommand{\CrossEntropy}[3][]{\mathcal{H} \Parentheses[#1]{\MidDoubleBar[#1]{#2}{#3}} }

\newcommand{\Diagonalise}[2][]{\diag \Parentheses[#1]{#2}}

% Vector or matrix
% The column specification works as follows:
% @{\,}         Left margin: \,
% *{#1}{        #1 times (optional parameter, default=1)
%   c@{\,\,}    Margin between entries: \,\,
% }
% @{\!}         Right margin: \,\,\! which is \,

%\newcommand{\Blocks}[2][1]{\left[ \begin{array}{@{\,}*{#1}{c@{\,\,}}@{\!}} #2 \end{array} \right]}
\newcommandtwoopt{\Blocks}[3][NoSizeOrColumns][NoSize]{%
	\ifthenelse{\equal{#1}{NoSizeOrColumns}}{%
		\def\BlocksDelimiterSize{auto}%
		\def\BlocksColumns{1}%
	}{%
		\ifthenelse{\equal{#2}{NoSize}}{%
			% No size given.
			\def\BlocksDelimiterSize{auto}%
			\def\BlocksColumns{#1}%
		}{%
			\def\BlocksDelimiterSize{#1}%
			\def\BlocksColumns{#2}%
		}%
	}%
	\SquareBrackets[\BlocksDelimiterSize]{
		\begin{array}{@{\,}*{\BlocksColumns}{c@{\,\,}}@{\!}}
			#3
		\end{array}
	}
}

% Probability
\newcommand{\Probability}[2][]{P \Parentheses[#1]{#2}}
\newcommand{\ProbabilityGiven}[3][]{P \Parentheses[#1]{\MidBar[#1]{#2}{#3}}}
\newcommand{\ProbabilityDistribution}[2][p]{#1\Parentheses{#2}}
%\newcommand{\ProbabilityDistributionGiven}[3][p]{#1 \Parentheses{\MidBar{#2}{#3}}}
\newcommand{\Expectation}[2][]{\ExpectationSymbol \CurlyBrackets[#1]{#2}}
\newcommand{\ExpectationUnder}[3][]{\ExpectationSymbol_{#2} \CurlyBrackets[#1]{#3}}
\newcommand{\ExpectationGiven}[3][]{\ExpectationSymbol \CurlyBrackets[#1]{\MidBar[#1]{#2}{#3}}}

\newcommandtwoopt{\ProbabilityDistributionGiven}[4][p][]{#1 \Parentheses[#2]{\MidBar[#2]{#3}{#4}}}

\newcommand{\DiracDelta}[2][]{\delta \Parentheses[#1]{#2}}
\newcommand{\KroneckerDelta}[2]{\delta \Parentheses{#1 - #2}}

%\newcommand{\UniformSymbol}{\mathcal{U}}
%\newcommand{\Uniform}[3][]{\UniformSymbol\Parentheses[#1]{#2, #3}}
\newcommand{\UniformSymbol}{\mathrm{Unif}}
\newcommand{\Uniform}[3][]{\UniformSymbol\SquareBrackets[#1]{#2, #3}}

\newcommand{\NormalSymbol}{\mathcal{N}}
\newcommand{\NormalV}[4][]{\NormalSymbol \Parentheses[#1]{%
    #2 ;\, #3 , \, #4%
}}
% \Normal[size][variable]{mean}{covariance}
% \Normal[variable]{mean}{covariance}
% \Normal{mean}{covariance}
\newcommandtwoopt{\Normal}[4][NoSizeNorVariable][NoSize]{%
	\ifthenelse{\equal{#1}{NoSizeNorVariable}}{%
		\def\NormalDelimiterSize{auto}%
		\def\NormalVariable{}%
	}{%
		\ifthenelse{\equal{#2}{NoSize}}{%
			% No size given.
			\def\NormalDelimiterSize{auto}%
			\def\NormalVariable{#1}%
		}{%
			\def\NormalDelimiterSize{#1}%
			\def\NormalVariable{#2}%
		}%
	}%
	\ifthenelse{\equal{\NormalVariable}{}}{%
	    \NormalSymbol %
	    \Parentheses[\NormalDelimiterSize]{#3, #4}%
    }{%
        \NormalV[\NormalDelimiterSize]{\NormalVariable}{#3}{#4}%
%		\NormalVariable \,;\, #3 \, , \, #4%
	}%
}



% Variable size delimiters

% \Delimiters[Bigg]{(}{text}{)}
\newcommand{\Delimiters}[4][auto]{%
	\ifthenelse{\equal{#1}{normal}}{%
		#2%
		#3%
		#4
	}{%
	\ifthenelse{\equal{#1}{big}}{%
		\big#2%
		#3%
		\big#4%
	}{%
	\ifthenelse{\equal{#1}{Big}}{%
		\Big#2%
		#3%
		\Big#4%
	}{%
	\ifthenelse{\equal{#1}{bigg}}{%
		\bigg#2%
		#3%
		\bigg#4%
	}{%
	\ifthenelse{\equal{#1}{Bigg}}{%
		\Bigg#2%
		#3%
		\Bigg#4%
	}{%
	    % Somehow the automatic setting for delimiter height adds \,
	    % around the delimiters. Undo with \!
		\!\left#2%
		#3%
		% There is sometimes space behind \right#4, but this is usually
		% no a problem, and there is no space when followed by & in an align
		% environment, which is the most common situation.
		% Therefore, the negative space here is commented out:
		\right#4%\!%
	}}}}}%
}

% \Separator[Bigg]{text}{\|}{text}
\newcommand{\Separator}[4][auto]{%
	\ifthenelse{\equal{#1}{normal}}{%
		#2%
		#3%
		#4
	}{%
	\ifthenelse{\equal{#1}{big}}{%
		#2%
		\big#3%
		#4%
	}{%
	\ifthenelse{\equal{#1}{Big}}{%
		#2%
		\Big#3%
		#4%
	}{%
	\ifthenelse{\equal{#1}{bigg}}{%
		#2%
		\bigg#3%
		#4%
	}{%
	\ifthenelse{\equal{#1}{Bigg}}{%
		#2%
		\Bigg#3%
		#4%
	}{%
		\!\left.%
		#2%
		\vphantom{#4}%
		\right#3\!%
		#4%
	}}}}}%
}

% Symbols

\newcommand{\NaturalNumbers}{\mathbb{N}}

\makeatletter

% If #1 is Latin, #2{#1}{<uppercase version of #1>}
% If #1 is Greek, #3{#1}{<uppercase version of #1>}
\newcommand{\ApplyLatinGreek}[3]{%
	\ifthenelse{\equal{#1}{\alpha}}{%
		#3{\alpha}{A}%
	}{%
	\ifthenelse{\equal{#1}{\eta}}{%
		#3{\eta}{H}%
	}{%
	\ifthenelse{\equal{#1}{\theta}}{%
		#3{\theta}{\Theta}%
	}{%
	\ifthenelse{\equal{#1}{\lambda}}{%
		#3{\lambda}{\Lambda}%
	}{%
	\ifthenelse{\equal{#1}{\mu}}{%
		#3{\mu}{\Mu}%
	}{%
	\ifthenelse{\equal{#1}{\sigma}}{%
		#3{\sigma}{\Sigma}%
	}{%
	\ifthenelse{\equal{#1}{\phi}}{%
		#3{\phi}{\Phi}%
	}{%
	\ifthenelse{\equal{#1}{\psi}}{%
		#3{\psi}{\Psi}%
	}{%
	\ifthenelse{\equal{#1}{\omega}}{%
		#3{\omega}{\Omega}%
	}{%
		#2{#1}{\MakeUppercase{#1}}%
	}}}}}}}}}%
}

\newcommand{\mathbfFirst}[2]{\mathbf{#1}}
\newcommand{\bmFirst}[2]{\bm{#1}}
\newcommand{\Second}[2]{#2}
\newcommand{\mathbfSecond}[2]{\mathbf{#2}}
\newcommand{\bmSecond}[2]{\bm{#2}}

% Turn a symbol into an uppercase version even if it's Greek.
\newcommand{\SequenciseSymbol}[1]{%
%    \ApplyLatinGreek{#1}{\Second}{\Second}%
    \ApplyLatinGreek{#1}{\mathbfFirst}{\bmFirst}%
}

% Turn a symbol into an uppercase bold version even if it's Greek.
\newcommand{\MatriciseSymbol}[1]{%
    \ApplyLatinGreek{#1}{\mathbfSecond}{\bmSecond}%
}

% Turn a symbol into an bold version even if it's Greek.
\newcommand{\VectoriseSymbol}[1]{%
    \ApplyLatinGreek{#1}{\mathbfFirst}{\bmFirst}%
}

% Turn a symbol into an uppercase version even if it's Greek.
\newcommand{\CountiseSymbol}[1]{%
    \ApplyLatinGreek{#1}{\Second}{\Second}%
}

% Turn a symbol into a capitalised caligraphic version.
\newcommand{\AggregatiseSymbol}[1]{%
	\mathcal{\MakeUppercase{#1}}%
}

\define@key{symbol}{Matrix}[]{%
	\def\symbol@type{\MatriciseSymbol}%
}
\define@key{symbol}{Sequence}[]{%
	\def\symbol@type{\SequenciseSymbol}%
}
\define@key{symbol}{Vector}[]{%
	\def\symbol@type{\VectoriseSymbol}%
}
\define@key{symbol}{Scalar}[]{%
	\def\symbol@type{}%
}
\define@key{symbol}{Count}[]{%
	\def\symbol@type{\CountiseSymbol}%
}
\define@key{symbol}{Aggregate}[]{%
	\def\symbol@type{\AggregatiseSymbol}%
}
\define@key{symbol}{Space}[]{%
	\def\symbol@type{\AggregatiseSymbol}%
}
\define@key{symbol}{Set}[]{%
	\def\symbol@type{\AggregatiseSymbol}%
}

\newcommand{\FrequentiseSymbol}[1]{%
	\MakeUppercase{#1}%
}

\define@key{symbol}{approximate}[]{%
	\def\symbol@modifier{\widetilde}%
}
\define@key{symbol}{estimate}[]{%
	\def\symbol@modifier{\hat}%
}
\define@key{symbol}{normalised}[]{%
	\def\symbol@modifier{\overline}%
}
\define@key{symbol}{resampled}[]{%
	\def\symbol@modifier{\hat}%
}

\define@key{symbol}{iteration}[\Iteration]{%
	\patchcommand\symbol@superscriptfirst{}{(#1)}%
}
\define@key{symbol}{number}[i]{%
	\patchcommand\symbol@superscriptfirst{}{(#1)}%
}

\define@key{symbol}{inverse}[{-1}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
\define@key{symbol}{square}[{2}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
\define@key{symbol}{cube}[{3}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
\define@key{symbol}{transpose}[\mathsf{T}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
% An inverse and a transpose at once: ^{-T}
\define@key{symbol}{inverseTranspose}[\mathsf{-T}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
% Hack to keep T's from floating off into space
\define@key{symbol}{innerTranspose}[\mathsf{T}]{%
	\patchcommand\symbol@superscriptsecond{}{\mathllap{#1}}%
}

\define@key{symbol}{index}[\Index]{%
	\patchcommand\symbol@subscriptsecond{}{#1}%
}

\newcommand{\Symbol}[3][]{%
	%%%%% Initialise variables
	\def\symbol@order{}%
	\def\symbol@superscriptfirst{}%
	\def\symbol@superscriptsecond{}%
	\def\symbol@subscriptfirst{}%
	\def\symbol@subscriptfirst@previous{}%
	\def\symbol@subscriptsecond{}%
	\def\symbol@type{}%
	\def\symbol@modifier{}%
	\def\symbol@following{}%
	% Defaults
	\setkeys{symbol}{#1}%
	\setkeys{symbol}{#3}%
	\def\symbol@appearance{\begingroup%
	    \symbol@modifier{\symbol@type{#2}}\endgroup%
	}%
	\patchcommand\symbol@superscriptfirst{\symbol@order}{}%
	%%%%%%% Super- and subscripts
	\ifthenelse{\equal\symbol@superscriptfirst{}}{%
		% No entry for \symbol@superscriptfirst;
		% move \symbol@superscriptsecond to \symbol@superscriptfirst.
		\let\symbol@superscriptsecondcopy\symbol@superscriptsecond%
		\patchcommand\symbol@superscriptfirst{}{\symbol@superscriptsecondcopy}%
		\def\symbol@superscriptsecond{}%
	}{}%
	\ifthenelse{\equal\symbol@subscriptfirst{}}{%
		% No entry for \symbol@subscriptfirst
		% move \symbol@subscriptsecond to \symbol@subscriptfirst.
		\let\symbol@subscriptsecondcopy\symbol@subscriptsecond%
		\patchcommand\symbol@subscriptfirst{}{\symbol@subscriptsecondcopy}%
		\def\symbol@subscriptsecond{}%
	}{}%
	\ifthenelse{\equal{\symbol@superscriptsecond}{}}%
	{%
		% If \symbol@superscriptsecond is empty
		\ifthenelse{\not{\equal{\symbol@subscriptsecond}{}}}%
		{%
			% use a comma
			\let\symbol@subscriptsecondcopy\symbol@subscriptsecond%
			\patchcommand\symbol@subscriptfirst{}{,\symbol@subscriptsecondcopy}%
			\def\symbol@subscriptsecond{}%
		}{}%
	}{%
		% If \symbol@superscriptsecond is non-empty
		\ifthenelse{\not{\equal{\symbol@subscriptsecond}{}}}%
		{%
			% use a comma
			\patchcommand\symbol@subscriptfirst{}{,}%
		}{}%
	}%
	%%%%%%% Output
	\def\symbol@first{%
		{\symbol@appearance}%
    	{\symbol@following}%
			\ifthenelse{\equal{\symbol@subscriptfirst}{}}{}%
				{_{\symbol@subscriptfirst}}%
			\ifthenelse{\equal{\symbol@superscriptfirst}{}}{}%
				{^{\symbol@superscriptfirst}}%
		}%
	\ifthenelse{\equal{\symbol@subscriptsecond\symbol@superscriptsecond}{}}%
		% No second-level entries
%		{\mbox{$\symbol@first$}}%
		{\symbol@first}%
		{%
			{\mbox{$\symbol@first$}}%
			\ifthenelse{\equal{\symbol@subscriptsecond}{}}{}%
				{_{\symbol@subscriptsecond}}%
			\ifthenelse{\equal{\symbol@superscriptsecond}{}}{}%
				{^{\symbol@superscriptsecond}}%
		}%
}

\makeatother

\newcommand{\Nothing}[1][]{%
	\Symbol[Matrix]{}{#1}%
}

\newcommand{\TransposeOf}[1]{%
	\Symbol{{#1}}{transpose}%
}
\newcommand{\InverseOf}[1]{%
	\Symbol{{#1}}{inverse}%
}
\newcommand{\SquareOf}[1]{%
	\Symbol{#1}{square}%
}
\newcommand{\IndexOf}[3][]{%
	\Symbol{#2}{index=#3, #1}%
}

\newcommand{\Zeros}[1][]{%
	\Symbol[Vector]{0}{#1}%
}
\newcommand{\Ones}[1][]{%
	\Symbol[Vector]{1}{#1}%
}

\newcommand{\DistributionSymbol}{p}
\newcommand{\Distribution}[1][]{%
	\Symbol{\DistributionSymbol}{#1}%
}



==> poster/symbols.tex <==
\usepackage{keyval}
\usepackage{patchcmd}
\usepackage{ifthen}
\usepackage{bm}

\input{math_notation}

%%%%%%%%%%%%
% Non-general things

%\usepackage{tipa}
%\newcommand{\PhoneExample}{\textipa{\ae}}
%% For retaining \! in math mode:
%\tipasafemode
\newcommand{\PhoneExampleOne}{ei}%\textsc{i}}
\newcommand{\PhoneExampleTwo}{t}

\newcommand{\WordIndexSymbol}{i}
\newcommand{\WordIndex}[1][]{%
	\Symbol[Scalar]{\WordIndexSymbol}{#1}%
}
\newcommand{\VocabularyWordSymbol}{v}
\newcommand{\VocabularyWord}[1][]{%
	\Symbol[Scalar]{\VocabularyWordSymbol}{#1}%
}
\newcommand{\VocabularyIndexSymbol}{j}
\newcommand{\VocabularyIndex}[1][]{%
	\Symbol[Scalar]{\VocabularyIndexSymbol}{#1}%
}

\newcommand{\SegmentSymbol}{s}
\newcommand{\Segment}[1][]{%
	\Symbol[Scalar]{\SegmentSymbol}{#1}%
}

\newcommand{\StartNodeName}{\text{start}}
\newcommand{\EndNodeName}{\text{end}}
\DeclareMathOperator*{\Forward}{forwd}
\DeclareMathOperator*{\Backward}{backwd}

\newcommand{\SemiringPlus}{\oplus}
\newcommand{\SemiringTimes}{\otimes}

\newcommand{\LanguageModelSize}{L}


\makeatletter

\define@key{symbol}{Automaton}[]{%
	\def\symbol@type{\AggregatiseSymbol}%
}

\makeatother

\newcommand{\GradientSymbol}{\nabla}
\newcommand{\Gradient}[1][]{%
	\Symbol[Scalar]{\GradientSymbol}{#1}%
}

\newcommand{\TransducerComposition}{\circ}

\newcommand{\SubPhoneAutomatonSymbol}{s}
\newcommand{\SubPhoneAutomaton}[1][]{%
	\Symbol[Automaton]{\SubPhoneAutomatonSymbol}{#1}%
}

\newcommand{\ObservationTransducerSymbol}{o}
\newcommand{\ObservationTransducer}[1][]{%
	\Symbol[Automaton]{\ObservationTransducerSymbol}{#1}%
}

\newcommand{\TrellisTransducerSymbol}{t}
\newcommand{\TrellisTransducer}[1][]{%
	\Symbol[Automaton]{\TrellisTransducerSymbol}{#1}%
}

\newcommand{\ArcSymbol}{e}
\newcommand{\Arc}[1][]{%
	\Symbol[Scalar]{\ArcSymbol}{#1}%
}

\newcommand{\PathSymbol}{\pi}
%\newcommand{\Path}{\Arc[Sequence]}
\newcommand{\Path}[1][]{%
	\Symbol[Scalar]{\PathSymbol}{#1}%
}

\newcommand{\WeightSymbol}{\sigma}
\newcommand{\Weight}[1][]{%
	\Symbol[Scalar]{\WeightSymbol}{#1}%
}
\newcommand{\WeightOf}[3][]{\Weight \SquareBrackets[#1]{ #2 ; #3}}

\newcommand{\PosteriorSymbol}{\gamma}
\newcommand{\Posterior}[1][]{%
	\Symbol[Scalar]{\PosteriorSymbol}{#1}%
}

\newcommand{\StartNodeSymbol}{p}
\newcommand{\StartNode}[1][]{%
	\Symbol[Scalar]{\StartNodeSymbol}{#1}%
}
\newcommand{\StartNodeOf}[2][]{\StartNode \SquareBrackets[#1]{ #2 }}

\newcommand{\EndNodeSymbol}{n}
\newcommand{\EndNode}[1][]{%
	\Symbol[Scalar]{\EndNodeSymbol}{#1}%
}
\newcommand{\EndNodeOf}[2][]{\EndNode \SquareBrackets[#1]{ #2 }}

\newcommand{\SemiringZero}{\overline 0}
\newcommand{\SemiringOne}{\overline 1}

\newcommand{\InputSymbolSymbol}{e}
\newcommand{\InputSymbol}[1][]{%
	\Symbol[Scalar]{\InputSymbolSymbol}{#1}%
}

\newcommand{\OutputSymbolSymbol}{o}
\newcommand{\OutputSymbol}[1][]{%
	\Symbol[Scalar]{\OutputSymbolSymbol}{#1}%
}

\newcommand{\LikelihoodSymbol}{\ell}
\newcommand{\Likelihood}[1][]{%
	\Symbol[Scalar]{\LikelihoodSymbol}{#1}%
}

\newcommand{\LikelihoodOf}[3][]{\Likelihood \SquareBrackets[#1]{ #2 ; #3}}
\newcommand{\LikelihoodOfAll}[2][]{\Likelihood \Parentheses[#1]{#2}}
\newcommand{\LikelihoodGiven}[3][]{\Likelihood \Parentheses[#1]{ #2 ; #3}}


%%%%%%%%%%%%%%

\newcommand{\TimeSymbol}{t}
\newcommand{\OtherTimeSymbol}{\tau}
\newcommand{\IndexSymbol}{i}
\newcommand{\WordSymbol}{w}

\newcommand{\VariableSymbol}{v}
\newcommand{\FactorSymbol}{f}
\newcommand{\FeatureSymbol}{\phi}
\newcommand{\NormalisationSymbol}{Z}

\newcommand{\ParameterSymbol}{\alpha}
\newcommand{\GenerativeParameterSymbol}{\lambda}

\newcommand{\StateSymbol}{s}
\newcommand{\ObservationSymbol}{o}

\newcommand{\EmptySymbol}{\epsilon}

\DeclareMathOperator*{\ParentsSymbol}{pa}

%%%%%% Implementations

\newcommand{\Parents}[1]{\ParentsSymbol \Parentheses{#1}}

\newcommand{\Time}[1][]{%
	\Symbol[Scalar]{\TimeSymbol}{#1}%
}
\newcommand{\TotalTime}[1][]{%
	\Symbol[Count]{\TimeSymbol}{#1}%
}
\newcommand{\TimeNum}[1][]{%
	\Symbol[Count]{\TimeSymbol}{#1}%
}
\newcommand{\OtherTime}[1][]{%
	\Symbol[Scalar]{\OtherTimeSymbol}{#1}%
}
\newcommand{\Index}[1][]{%
	\Symbol[Scalar]{\IndexSymbol}{#1}%
}

\newcommand{\Word}[1][]{%
	\Symbol[Scalar]{\WordSymbol}{#1}%
}

\newcommand{\State}[1][]{%
	\Symbol[Scalar]{\StateSymbol}{#1}%
}
\newcommand{\Observation}[1][]{%
	\Symbol[Scalar]{\ObservationSymbol}{#1}%
}

\newcommand{\Variable}[1][]{%
	\Symbol[Scalar]{\VariableSymbol}{#1}%
}
\newcommand{\Factor}[1][]{%
	\Symbol[Scalar]{\FactorSymbol}{#1}%
}
\newcommand{\Feature}[1][]{%
	\Symbol[Scalar]{\FeatureSymbol}{#1}%
}

\newcommand{\Normalisation}[1][]{%
	\Symbol[Scalar]{\NormalisationSymbol}{#1}%
}

\newcommand{\Parameter}[1][]{%
	\Symbol[Scalar]{\ParameterSymbol}{#1}%
}
\newcommand{\GenerativeParameter}[1][]{%
	\Symbol[Scalar]{\GenerativeParameterSymbol}{#1}%
}

\makeatletter

%\define@key{symbol}{velocity}[\mathsf{\Delta}]{%
\define@key{symbol}{velocity}[\Delta]{%
	\def\symbol@order{#1}%
}
\define@key{symbol}{acceleration}[\Delta^2]{%
	\def\symbol@order{#1}%
}

\define@key{symbol}{time}[\TimeSymbol]{%
	\ifthenelse{\equal{\symbol@subscriptfirst@previous}{symbol}}{%
		\patchcommand\symbol@subscriptfirst{}{_{#1}}%
	}{%
		\patchcommand\symbol@subscriptfirst{}{#1}%
	}%
}

\define@key{symbol}{best}[*]{%
	\patchcommand\symbol@superscriptfirst{}{#1}%
}

\define@key{symbol}{state}[\mathsf{\StateSymbol}]{%
	\patchcommand\symbol@subscriptfirst{}{#1}%
%	\def\symbol@subscriptfirst@previous{symbol}%
}
\define@key{symbol}{observation}[\mathsf{\ObservationSymbol}]{%
	\patchcommand\symbol@subscriptfirst{}{#1}%
	\def\symbol@subscriptfirst@previous{symbol}%
}

\define@key{symbol}{sequential}[\text{\textsf{seq}}]{%
	\patchcommand\symbol@superscriptfirst{}{#1}%
}
\define@key{symbol}{observational}[\text{\textsf{obs}}]{%
	\patchcommand\symbol@superscriptfirst{}{#1}%
}

\makeatother



==> poster/ucamcolor.tex <==
%--------------------------------------------------------
% Set up the Cambridge University Colours for use with
% xcolor
%--------------------------------------------------------

% Blue palette
% Pantone 284 C
\definecolor{lightBlue}{rgb}{0.4157 0.6784 0.8941}
% Pantone 285 C
\definecolor{coreBlue}{rgb}{0 0.4510 0.8118}
% Pantone 541 C
\definecolor{darkBlue}{rgb}{0 0.2341 0.4471}

% Orange palette
% Pantone 142 C
\definecolor{lightOrange}{rgb}{0.9373 0.7412 0.2784}
% Pantone 158 C
\definecolor{coreOrange}{rgb}{0.8902 0.4471 0.1333}
% Pantone 718 C
\definecolor{darkOrange}{rgb}{0.7843 0.3059 0}

% Green palette
% Pantone 583 C
\definecolor{lightGreen}{rgb}{0.6588 0.7059 0}
% Pantone 369 C
\definecolor{coreGreen}{rgb}{0.3451 0.6510 0.0941}
% Pantone 574 C
\definecolor{darkGreen}{rgb}{0.2627 0.3176 0.1451}

% Purple palette
% Pantone 5215 C
\definecolor{lightPurple}{rgb}{0.7098 0.5765 0.6078}
% Pantone 513 C
\definecolor{corePurple}{rgb}{0.5569 0.1451 0.5529}
% Pantone 669 C
\definecolor{darkPurple}{rgb}{0.2549 0.1765 0.3647}

% Teal palette
% Pantone 557 C
\definecolor{lightTeal}{rgb}{0.6392 0.7569 0.6784}
% Pantone 7466 C
\definecolor{coreTeal}{rgb}{0 0.7020 0.7451}
% Pantone 5473 C
\definecolor{darkTeal}{rgb}{0.0824 0.3961 0.4392}



==> sdc_jul11.tex <==

\section{Vehicle Motion Prediction}

We present the Shifts Vehicle Motion Prediction dataset to examine the implications of distributional shifts in self-driving vehicles. The area of autonomous vehicle (AV) technology is highly relevant for uncertainty and robustness research, as the safety requirements and the risks associated with any errors made are high. Furthermore, distributional shift is ubiquitous in the autonomous driving domain. Most self-driving companies concentrate their fleet in a limited number of locations and routes due to the large cost of operating in an incremental location. Therefore, fleets often face distributional shift when they begin operation at a new location, or even a new route in an existing location. It is thus important to transfer as much knowledge as possible from the old locations to the new one. It is also critical for a planning model to recognize when this transferred knowledge is insufficient upon encountering unfamiliar data, which could risk unpredictable and unsafe behavior. Uncertainty quantification therefore has potentially life-critical application in this domain. For example, when the model's predictive uncertainty reaches a particular threshold, the vehicle can exercise extra caution or even transfer control to the human driver \cite{michelmore2018evaluating}. 

The problem of motion prediction is among the most important in the autonomous driving domain and has recently drawn significant attention from both academia and industry \cite{alahi2016social, lee2017desire, gupta2018social, chai2019multipath, casas2019spatially, cui2019multimodal, phan2020covernet, gao2020vectornet, biktairov2020prank, casas2020implicit, liang2020learning, liu2021multimodal}. The task of Motion Prediction involves predicting the distribution over possible future states (positions) of agents (vehicles) around the self-driving car at a number of moments in time. As any vehicle, a self-driving vehicle needs a certain amount of time to change its speed, and sudden changes may be uncomfortable or even dangerous for its passengers. Therefore, in order to ensure a safe and comfortable ride, self-driving vehicles use motion planning modules to reason about where other vehicles might end up in a few seconds. The problem is additionally complicated by the fact that \emph{the future is inherently uncertain}.
For example, we cannot know the high-level navigational goals of other agents, or even their low-level tendency to turn right or left at a T-junction if they fail to indicate one way or another. In order for the planning module to make the right decision, this uncertainty must be precisely quantified.

Motion prediction is interesting not only due to its real-world application and the safety-critical nature of autonomous vehicle technology, but also because the predictions are both \emph{structured and continuous}. This poses further challenges in uncertainty estimation. Recently, ensemble-based uncertainty estimation for the related task of autonomous vehicle \emph{planning} was examined~\cite{filos2020can}, where a variance-based measure was proposed. However, there is still much potential for further development of informative measures of uncertainty in continuous structured prediction tasks, such as motion prediction.


\subsection{Dataset Description}


\begin{table}[htbp]
  \caption{A comparison of various motion prediction datasets. The Shifts Vehicle Motion Prediction dataset is the largest by number of scenes and total size in hours.}
  \label{table:sdc_dataset_comparison}
  \begin{center}
  \begin{small}
    \begin{tabular}{ l |cccccc }
      \toprule
       \multirow{2}{*}{Dataset} & \multirow{2}{*}{Scene Length (s)} &  \multicolumn{3}{c}{\# Scenes} & \multirow{2}{*}{Total Size (h)} & \multirow{2}{*}{Avg. \# Actors} \\ 
       & & Train & Val & Test & &  \\
       \midrule
            Argoverse  & 5 & 205,942 & 39,472 & 78,143 & 320 & 50 \\
            Lyft & 25 & 134,000 & 11,000 & 16,000 & 1,118 & 79 \\
            Waymo & 20 & 72,347 & 15,503 & 15,503 & 574 & - \\
            Shifts & 10 & 500,000 & 50,000 & 50,000 & 1,667 & 29 \\
      \bottomrule
    \end{tabular}
  \end{small}
  \end{center}
\end{table}

The dataset for the Vehicle Motion Prediction task was collected by the Yandex Self-Driving Group (SDG) fleet.
This is the largest vehicle motion prediction dataset released to date, containing 600,000 scenes (see \cref{table:sdc_dataset_comparison} for a comparison to other public datasets). We release this dataset under the CC BY NC SA 4.0 license. The dataset consists of scenes spanning six locations, three seasons, three times of day, and four weather conditions (cf. \cref{table:sdc_dataset_loc_season} and \ref{table:sdc_dataset_prec_tod}). Each of these conditions is available in the form of tags associated with every scene.
Each scene is 10 seconds long and is divided into 5 seconds of context features and 5 seconds of ground truth targets for prediction, separated by the time $T=0$. The goal of the task is to predict the movement trajectory of vehicles at time $T \in \left(0, 5\right]$ based on the information available for time $T \in \left[-5, 0\right]$. 
\begin{table}[htbp]
  \caption{The number of scenes in the Vehicle Motion Prediction dataset by location and season.}
  \label{table:sdc_dataset_loc_season}
  \begin{center}
  \begin{small}
    \begin{tabular}{ l |ccc }
      \toprule
Location & Train & Validation & Test \\
      \midrule
        Moscow & 450,504 & 30,505 & 30,534 \\
        Skolkovo & 6,283 & 2,218 & 2,956 \\
        Innopolis & 15,086 & 5,164 & 5,016 \\
        Ann Arbor & 19,349 & 8,290 & 6,617 \\
        Modiin & 3,502 & 2,262 & 1,555 \\
        Tel Aviv & 5,276 & 1,561 & 3,322 \\
            \bottomrule
    \end{tabular}
  \end{small}
  \quad
    \begin{small}
    \begin{tabular}{ l |ccc }
    \toprule
        Season & Train & Validation & Test \\
        \midrule
        Summer & 85,698 & 10,634 & 10,481 \\
        Autumn & 126,845 & 15,290 & 15,840 \\
        Winter & 287,457 & 24,076 & 23,679 \\
        Spring & 0 & 0 & 0 \\
    \bottomrule
    \end{tabular}
  \end{small}
  \end{center}
\end{table}

Each scene includes information about the state of dynamic objects (i.e., vehicles, pedestrians) and an HD map.
Each vehicle is described by its position, velocity, linear acceleration, and orientation (yaw, known up to $\pm\pi$).
A pedestrian state consists of a position vector and a velocity vector. All state components are represented in a common coordinate frame and sampled at 5Hz frequency by the perception stack running on the Yandex SDG fleet. The HD map includes lane information (e.g., traffic direction, lane priority, speed limit, traffic light association), road boundaries, crosswalks, and traffic light states, which are also sampled at 5Hz.\footnote{To made it easier to use this dataset, we provide utilities to render scene information as a feature map, which can be used as an input to a standard vision model (e.g., a ResNet \cite{resnet}). Our utilities represent each scene as a birds-eye-view image with each channel corresponding to a particular feature (e.g., a vehicle occupancy map) at a particular timestep. We also provide pre-rendered feature maps for every prediction request (cf. \cref{subsection:task_setup}) in the dataset, which are used to train the baseline models. The maps are $128 \times 128$ pixels in size with each pixel covering 1 square meter, have $17$ channels describing both HD map information and dynamic object states at time $T = 0$, and are centered with respect to the agent for which a prediction is being made. Researchers working with the dataset are free to use these feature maps, use the provided utilities to render another set of feature maps at different (earlier) timesteps, or construct their own scene representations from the raw data.}

The ground truth part of a scene contains future states of dynamic objects sampled at 5Hz for a total of $25$ state samples. Some objects might not have all $25$ states available due to occlusions or imperfections of the on-board perception system.
\begin{table}[htbp]
  \caption{The number of scenes in the Vehicle Motion Prediction dataset by precipitation and time of day.}
  \label{table:sdc_dataset_prec_tod}
  \begin{small}
    \begin{tabular}{ l |ccc }
      \toprule
Precipitation Type & Train & Dev & Eval \\
\midrule
No & 432,598 & 44,799 & 44,274 \\
Rain & 15,618 & 1,857 & 1,751 \\
Sleet & 15,210 & 1,082 & 990 \\
Snow & 36,574 & 2,262 & 2,985 \\
            \bottomrule
    \end{tabular}
  \end{small}
  \quad
    \begin{small}
    \begin{tabular}{ l |ccc }
      \toprule
Sun Phase & Train & Dev & Eval \\
\midrule
Astronomical Night & 171,867 & 13,164 & 13,113 \\
Daylight & 299,065 & 33,879 & 33,979 \\
Twilight & 29,068 & 2,957 & 2,908 \\
\bottomrule
    \end{tabular}
  \end{small}
\end{table}

A number of vehicles in the scene are labeled as \emph{prediction requests}. These are the vehicles that are visible at the most recent time $T=0$ in the context features part of a scene, and therefore would call for a prediction in a deployed system. 
For such vehicles we provide not only their future trajectories, but also a number of non--mutually exclusive tags, detailed in table~\ref{tab:trajectory_tags} describing the associated maneuver in more detail -- whether the vehicle is turning, accelerating, slowing down, etc. -- for a total of $10$ maneuver types. Note that some prediction requests may not have all $25$ state samples available.
We call prediction requests with fully-observed state \emph{valid} prediction requests and propose to evaluate predictions only on those.
\begin{table}[h]
  \caption{Number of actors maneuvers}
  \begin{center}
  \begin{small}
    \begin{tabular}{l | ccc}
\toprule
Maneuver type & train & validation & test \\
\midrule
Move left & 254843 & 25049 & 25820 \\
Move right & 322231 & 30074 & 30633 \\
Move forward & 5032724 & 395467 & 413920 \\
Move back & 54677 & 4811 & 4891 \\
Acceleration & 2473750 & 206977 & 215009 \\
Deceleration & 2050186 & 168550 & 174477 \\
Uniform movement & 6369920 & 566083 & 573033 \\
Stopping & 441619 & 38411 & 39336 \\
Starting & 739143 & 64986 & 65759 \\
Stationary & 4620678 & 433161 & 433576 \\
\bottomrule
    \end{tabular}
  \end{small}
  \end{center}\label{tab:trajectory_tags}
\end{table}

In order to study the effects of distributional shift, assess robustness to it and the ability of models to yields accurate uncertainty estimates, we partition this dataset such that there are `in-domain' data which are matched to the training set, and `out-of-domain' or `shifted' data which are mismatched to the training data. Furthermore, we provide a `development' set which acts as a validation set and an `evaluation set' which acts as the test set. For benchmarking and reporting baseline performance results, we define a ``canonical partitioning'' of the full dataset (cf. \cref{fig:sdc_partitioning}, \cref{table:sdc_partitioning}) as the following. The training, in-domain development, and in-domain evaluation data are taken from Moscow. Distributionally shifted development data is taken from Skolkovo, Modiin, and Innopolis. Distributionally shifted evaluation data is taken from Tel Aviv and Ann Arbor. In addition, we remove all cases of precipitation from the in-domain training, development, and test sets, while distributionally shifted datasets include precipitation. A full description of the canonical partitioning is described in \cref{fig:sdc_partitioning}. This partitioning will also be the one used in the Shifts Challenge.
\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figures/SDC_data_partition.png}
  \caption{The canonical partitioning of the Vehicle Motion Prediction dataset.}
  \label{fig:sdc_partitioning}
\end{figure}

\begin{table}[htbp]
  \caption{The number of scenes in the canonical dataset partitioning.}
  \label{table:sdc_partitioning}
  \begin{center}
  \begin{small}
    \begin{tabular}{ l | cc }
      \toprule
      Dataset Partition & In-Distribution & Distributionally Shifted  \\
      \midrule
            Train & 388,406 & - \\
            Development & 27,036 & 9,569 \\
            Evaluation & 26,865 & 9,939 \\
      \bottomrule
    \end{tabular}
  \end{small}
  \end{center}
\end{table}

\subsection{Task Setup} \label{subsection:task_setup}

Vehicle Motion Prediction is a complex task and needs to be described in detail.  We provide a training dataset $\mathcal{D}_\textup{train}=\{(\bm{x}_i, \bm{y}_i)\}_{i = 1}^{N}$ of time-profiled ground truth trajectories (i.e., plans) $\bm{y}$ paired with high-dimensional observations (features) $\bm{x}$ of the corresponding scenes. Each $\bm{y} = (s_1, \dots, s_T)$ corresponds to the trajectory of a given vehicle observed through the SDG perception stack. Each state $s_t$ corresponds to the x- and y-displacement of the vehicle at timestep $t$, s.t. $\bm{y} \in \mathbb{R}^{T \times 2}$. We consider the performance of models on development and evaluation datasets $\mathcal{D}^{j}_\textup{dev}=\{(\bm{x}_i, \bm{y}_i)\}_{i = 1}^{M_j}$. and $\mathcal{D}^{j}_\textup{eval}=\{(\bm{x}_i, \bm{y}_i)\}_{i = 1}^{M_j}$. See \cref{fig:sdc_model} for a depiction of the task. 

\textbf{Prediction Requests.} 
There are $N$ ($M_j$) prediction requests in the training dataset (evaluation datasets), with many requests for each scene corresponding to the many different vehicle trajectories observed. For example, in the canonical partition of the data, there are 388,406 scenes in the training dataset (Moscow, no precipitation), and 5,649,675 valid prediction requests.

Models can be trained to make use of ground truth trajectories that contain occlusions (i.e., prediction requests that are not valid) during training, such as through linear interpolation of missing steps. However, for the benchmarks considered in this work, both training and evaluation are done using only the fully observed ground truth trajectories.

Next, we describe the two levels of uncertainty quantification that we consider for each prediction request in the proposed task: per-trajectory and per--prediction request uncertainty scores.

\textbf{Per-Trajectory Confidence Scores.} Like machine translation, motion prediction is an inherently multi-modal task. A motion prediction model can produce a different number of sampled trajectories (plans) $D_i$ for each input $\bm{x}_i$; in other words, for two inputs $\bm{x}_i, \bm{x}_j$ with $i \neq j$, $D_i$ and $D_j$ can differ.
As a justification, consider that in a certain context, multiple trajectories may be desirable to capture multi-modality (e.g., the vehicle of interest is at a T-junction), and in others a single or fewer trajectories would be sufficient (e.g., the vehicle is clearly proceeding straight). In our task, we expect a stochastic model to accompany its $D_i$ predicted trajectories on a given input $\bm{x}_i$ with scalar, normalized, per-trajectory confidence scores $c_i^{(d)}, d \in \{1, \dots D_i\}$.  These provide an ordering of the plausibility of the various trajectories predicted for a given input. The scores must be non-negative and sum to $1$ (i.e., form a valid probability distribution). 
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/motion_prediction_model_1.png}
  \caption{Diagram of the Vehicle Motion Prediction task. Models take as input a single scene context $\bm{x}$ composed of static (HD map) and time-dependent input features, and predict trajectories $\{\bm{y}^{(d)} \mid d \in 1, \dots, D\}$ with corresponding per-trajectory confidence scores $\{\bm{c}^{(d)} \mid d \in 1, \dots, D\}$, as well as a single per--prediction request uncertainty score $C$.}
  \label{fig:sdc_model}
\end{figure}

\textbf{Per-Prediction Request Uncertainty Measure.}
We also expect models to produce a scalar uncertainty estimates corresponding to each prediction request input $\bm{x}_i$.
For example, on evaluation dataset $\mathcal{D}^{j}_\textup{eval}$, we have $M_j$ per-prediction request uncertainty estimates $\{C_i \mid i \in 1, \dots, M_j\}$. These correspond to the model's uncertainty in making any trajectory prediction for the agent of interest. In a real-world deployment setting, a self-driving vehicle would associate a high per-prediction request uncertainty estimates with a scene context that is particularly unfamiliar or high-risk. %For the purposes of metrics performing retention over prediction requests (described in \cref{subsection:performance_metrics}), only a relative ordering of prediction requests is needed. Therefore we can easily convert between confidence and uncertainty by negating the scores.

Next, we will describe standard motion prediction performance metrics, followed by confidence-aware metrics which reward models with well-calibrated uncertainty.

\subsection{Metrics}

\textbf{Standard Performance Metrics.}
We assess the performance of a motion prediction system using several standard metrics.

The average displacement error (ADE) measures the quality of a predicted trajectory $\bm{y}$ with respect to the ground truth trajectory $\bm{y}^*$ as
\begin{equation}
    \text{ADE}(\bm{y}) \coloneqq \frac{1}{T} \sum_{t = 1}^T \left\lVert s_t - s^*_t \right\rVert_2,
\label{eq:ade}
\end{equation}
where $\bm{y} = (s_1, \dots, s_T)$. Analogously, the final displacement error
\begin{equation}
    \text{FDE}(\bm{y}) \coloneqq \left\lVert s_T - s^*_T \right\rVert_2,
\label{eq:fde}
\end{equation}
measures the quality at the last timestep.

Stochastic models define a predictive distribution $q(\bm{y} \mid \bm{x}; \bm{\theta})$, and can therefore be evaluated over the $D$ trajectories sampled for a given input $\bm{x}$. For example, we can measure an aggregated ADE over $D$ samples with
\begin{equation}
    \text{aggADE}_D(q) \coloneqq \underset{\{\bm{y}\}_{d = 1}^{D} \sim q(\bm{y} \mid \bm{x})}{\oplus} \text{ADE}(\bm{y}^{d}),
\label{eq:agg_ade}
\end{equation}
where $\oplus$ is an aggregation operator, e.g., $\oplus = \min$ recovers the minimum ADE ($\text{minADE}_{D}$) commonly used in evaluation of stochastic motion prediction models \cite{filos2020can, phan2020covernet}. We consider minimum and mean aggregation of the average displacement error (minADE, avgADE), as well as of the final displacement error (minFDE, avgFDE).

\textbf{Per-Trajectory Confidence-Aware Metrics.}
A stochastic model used in practice for motion prediction must ultimately ``decide'' on a particular predicted trajectory for a given prediction request. We may make this decision by selecting for evaluation the predicted trajectory with the highest per-trajectory confidence score. In other words, given per-trajectory confidence scores $\{c^{(d)} \mid d \in 1, \dots, D\}$ we select the top trajectory $y^{(d^{*})}, d^* = \underset{d}{\arg \max}\ c^{(d)}$, and measure the decision quality using ``top1'' ADE and FDE metrics, e.g.,
\begin{equation}
    \text{top1ADE}_D(q) \coloneqq \text{ADE}(\bm{y}^{(d^*)}).
\label{eq:top1_ade}
\end{equation}

We may also wish to assess the quality of the relative weighting of the $D$ trajectories with their corresponding per-trajectory confidence scores $c^{(d)}$. This is accomplished with a weighted metric
\begin{equation}
    \text{weightedADE}_D(q) \coloneqq \sum_{d \in D} c^{(d)} \cdot \text{ADE}(\bm{y}^{(d)}).
\label{eq:weighted_ade}
\end{equation}
The top1FDE and weightedFDE metrics follow analogously to the above.

\textbf{Per-Prediction Request Confidence-Aware Metrics.}
In addition to making a decision amongst many possible trajectories in a particular situation, a motion planning agent should know when, in general, any trajectories it predicts will be inaccurate (e.g., due to unfamiliarity of the setting, or inherent ambiguity in the path of the vehicle for which a prediction is requested). We evaluate the quality of uncertainty quantification jointly with robustness to distributional shift using the retention-based metrics described in section~\ref{sec:metrics}, using the per-prediction request uncertainty estimates to determine retention order. Note that each retention curve is plotted with respect to a particular error metric above (e.g., we consider AUC for retention with respect to weightedADE). Additionally, we also assess whether the per-prediction uncertainty estimates can be used to discriminated between in-domain and shifted scenes. Here, quality is assessed via area under an ROC curve.


















\subsection{Baselines Results} \label{subsection:sdc_baseline_results}
%\subsection{Baseline: Robust Imitative Planning}

\textbf{Robust Imitative Planning.} As our baseline we will consider Robust Imitative Planning (RIP)~\cite{filos2020can}, where an ensemble of probabilistic models is used to stochastically generate multiple predictions for a given prediction request. We adapt the method to produce uncertainty estimates at our two desired levels of granularity: per-trajectory and per--prediction request.
In detail, we use the following approach for trajectory and confidence score generation.
\begin{enumerate}[label=\textbf{\arabic*})]
    \item \textbf{Trajectory Generation.} Given a scene input $\bm{x}$, $K$ ensemble members generate $G$ trajectories.\footnote{In practice, each ensemble member generates the same number of trajectories $Q$, s.t. $G = K \cdot Q$.}
    \item \textbf{Trajectory Scoring.} We score each of the $G$ trajectories by computing a log probability under each of the $K$ trained likelihood models. 
    \item \textbf{Per-Trajectory Confidence Scores.} We aggregate the $G \cdot K$ resulting log probabilities to $G$ scores using a per-trajectory aggregation operator $\oplus_{\text{trajectory}}$.\footnote{For example, applying a $\min$ aggregation is informed by robust control literature \cite{wald1939contributions} in which we aim to optimize for the worst-case scenario, as measured by the log-likelihood of the ``most pessimistic'' model for a given trajectory.} 
    By aggregating over the log-likelihood estimates sampled from the model posterior (i.e., contributed by each ensemble member), we obtain a robust score for each of the $G$ trajectories \cite{filos2020can}.
    \item \textbf{Per--Prediction Request Uncertainty Score.} We aggregate the $G$ per-trajectory scores to a single score $C$ using the aggregator $\oplus_{\text{pred-req}}$. This value conveys ensemble's uncertainty estimate for a given scene context and a particular prediction request.
    \item \textbf{Trajectory Selection.} Among the $G$ trajectories, the RIP ensemble produces the top $D$ trajectories as determined by their corresponding $G$ per-trajectory confidence scores, where $D$ is a hyperparameter.
   \item \textbf{Confidence Reporting.} We obtain scores $c^{(d)}$ by applying a \texttt{softmax} to the $D$ top per-trajectory  confidence scores. We report these $c^{(d)}$ and $C$ (computed in step \textbf{4}) as our final per-trajectory  confidence scores and per--prediction request uncertainty score, respectively.
\end{enumerate}

To summarize, our implementation of RIP for motion prediction produces $D$ trajectories and corresponding normalized per-trajectory scores $\{c^{(d)} \mid d \in 1, \dots, D\}$, as well as an aggregated uncertainty $C$ for the overall prediction request. 

\textbf{Backbone Likelihood Model.} We consider two different model classes as ensemble members: a simple behavioral cloning agent with a Gated Recurrent Unit decoder (BC) \cite{cho2014learning, codevilla2018end} and a Deep Imitative Model (DIM) \cite{rhinehart2018deep} with an autoregressive flow decoder \cite{rezende2016variational}, following \cite{filos2020can}.
In both cases, we model the likelihood of a trajectory $\bm{y}$ in context $\bm{x}$ to come from an expert (i.e., from the distribution of ground truth trajectories), with learnable parameters $\bm{\theta}$, as
\begin{equation}
\begin{split}
q(\bm{y} \mid \bm{x}; \bm{\theta}) & = \prod_{t = 1}^T p(s_t \mid \bm{y}_{<t}, \bm{x}; \bm{\theta})\ = \prod_{t = 1}^{T} \mathcal{N}(s_t; \mu(\bm{y}_{<t}, \bm{x}; \bm{\theta}), \Sigma(\bm{y}_{<t}, \bm{x}; \bm{\theta})),
\end{split}
\label{eq:sdc_likelihood_model}
\end{equation}
where $\mu(\cdot; \bm{\theta})$ and $\Sigma(\cdot; \bm{\theta})$ are two heads of a recurrent neural network with shared torso. 
Hence we assume that the conditional densities are normally distributed, and learn those parameters through maximum likelihood estimation.
Notably, for the BC model, we found that conditioning on samples $\hat{\bm{y}}_{<t}$ instead of ground truth values $\bm{y}_{<t}$ (where usage of ground truth is often referred to as teacher forcing in RNN literature) significantly improved performance across all datasets and metrics.

% We no longer use predictive variance for the scores.

% * We obtain the per-trajectory confidence scores by computing the disagreement between the qualities of each trajectory under models sampled from the posterior $p(\bf{\theta}, \mathcal{D})$. 
%     * In particular, for each of the $K \cdot D$ predicted trajectories $\bf{y}$, we compute the variance of the imitation prior with respect to the model posterior as
% \begin{equation}
%     u(\bf{y}) \coloneqq \text{Var}_{p(\bf{\theta}|\mathcal{D})}[\log q(\bf{y}|\bf{x}; \bf{\theta})]
% \label{eq:pred_var}
% \end{equation}    
% We can negate this predictive variance to obtain a per-trajectory confidence, i.e., $c_d = -u(\bf{y}^{d})$. 
% To obtain a per-scene confidence, we simply average confidences across all predicted trajectories for a scene, i.e., 
% \begin{equation}
%     C_M = \frac{1}{KD} \sum_{d = 1}^{KD} c_d
% \label{eq:scene_confidence}
% \end{equation}

% simply reporting the aggregated log imitation prior (i.e., in the Worst Case Model setting, the lowest log imitation prior score among the K models, for each of the $K \cdot D$ plans. 

\textbf{Setup.} We report performance of the two RIP variants -- BC and DIM -- on development (\texttt{dev}) and evaluation (\texttt{eval}) datasets in both in-distribution and distributionally shifted settings.
With both backbone model classes we use $K = 5$ ensemble members, train with learning rate 1e-4, use a cosine annealing LR schedule with 1 epoch warmup, and use gradient clipping at 1. 
We sample $Q = 10$ trajectories from each of the ensemble members, for a total of $G = 50$ trajectories to be scored.
We use ``Lower Quartile'' aggregation for both the per-trajectory aggregation operator $\oplus_{\text{plan}}$ and the per--prediction request aggregation operator $\oplus_{\text{pred-req}}$, reporting the mean minus the standard deviation $\mu - \sigma$ of the scores taken as input. This reflects the intuition to assign a high score to a trajectory when the ensemble members assign it a high score on average, and tend to be certain (have a low standard deviation) in their scoring.
We fix the RIP ensemble to produce the top $D = 5$ trajectories as ranked by their per-trajectory confidence score.




\textbf{Aggregate Results.} See \cref{table:sdc_performance} for the performance of the two RIP variants across the \texttt{dev} and \texttt{eval} datasets. We observe that RIP (BC) consistently performs better than RIP (DIM) on the per-trajectory confidence weighted metrics (weightedADE and weightedFDE), and RIP (DIM) outperforms RIP (BC) on minADE and minFDE.
This result might occur if DIM has higher predictive variance. In such a case, DIM might be more effective in modeling multimodality, and therefore would tend to produce at least one high accuracy trajectory on more scenes, improving performance on \texttt{min} aggregation metrics. On the other hand, for ``obvious" scenes, DIM might then produce unnecessarily complicated trajectories which would be reflected in poor performance on \texttt{weighted} aggregation metrics.

For the metrics which consider \emph{all datapoints} in the evaluation datasets, as opposed to the AUC of the retention curve, or observing the curve at a specific threshold -- in other words, the minADE, weightedADE, minFDE, and weightedFDE metrics -- we observe that in all cases the performance on the distributionally shifted dataset is worse than that on the in-distribution dataset.
However, interestingly, we find that on the retention metrics (e.g., AUC-weightedADE), the performance on the distributionally shifted \texttt{dev} dataset exceeds that on the in-distribution \texttt{dev} dataset: for example, AUC-weightedADE for DIM on in-distribution \texttt{dev} achieves AUC $= 0.488$, versus AUC $= 0.424$ for shifted \texttt{dev}, where lower is better. 
One potential explanation is that there are certain examples on which the model performs particularly poorly in the shifted datasets, and that on retention tasks, their disproportionate contribution to the loss metric can be mitigated with well-calibrated uncertainty (a particularly high uncertainty on those examples). 

\begin{table}[p]
    \centering
    \caption{Predictive Performance of the two RIP variants -- behavioral cloning (BC) \cite{codevilla2018end} and Deep Imitative Model (DIM) \cite{rhinehart2018deep} -- on the in-distribution and distributionally shifted development and evaluation datasets. The \emph{Full Dev} (\emph{Full Eval}) sections contain losses computed over the in-distribution and distributionally shifted development (evaluation) datasets jointly. The top performer between the two variants for each metric and dataset split is \textbf{bolded}.
    See \cref{subsection:sdc_baseline_results} for setup details.}
    \label{table:sdc_performance}
\vspace{0.1in}
\resizebox{1\textwidth}{!}{%
    \begin{tabular}{@{}ll|ccc|ccc|ccc|ccc}
        \toprule
          \multirow{2}*{Dataset} &  \multirow{2}*{Model} & \multicolumn{3}{c|}{\text{minADE} $\downarrow$} & \multicolumn{3}{c|}{\text{weightedADE} $\downarrow$} & \multicolumn{3}{c|}{ \text{minFDE} $\downarrow$} &  \multicolumn{3}{c}{\text{weightedFDE} $\downarrow$}\\
          & & In & Shifted & Full & In & Shifted & Full & In & Shifted & Full & In & Shifted & Full   \\
        \midrule
        \multirow{3}*{Dev}   & \text{BC, LQ, K=1} & 0.810 &  0.945 &  0.826& 1.085 & 1.238 & 1.104 & 1.695 & 2.075 & 1.741 & 2.363 & 2.757 & 2.410 \\
        &\text{BC, LQ, K=5} & 0.766 & 0.889 &  0.781 & 1.018 & 1.139 & 1.032 & 1.618 & 1.982 & 1.662 & 2.216 &2.554 & 2.256 \\
        & \text{DIM, LQ, K=1} & 0.749 & 0.831 &  0.759  & 1.493 & 1.587  & 1.504 & 1.507 & 1.753 & 1.537  & 3.421 &3.660 &3.450  \\
        % \text{DIM, LQ, K=5} & \bf{0.721} & 0.788  &  0.729  & 1.399 & 1.470 & 1.407 & \bf{1.487} & 1.705 &  1.514 & 3.201 & 3.397& 3.225  \\
        \midrule
  \multirow{3}*{Eval}  & \text{BC, LQ, K=1} & 0.823 & 1.074  &  0.874  & 1.103 &  1.401  & 1.163   & 1.720 & 2.398  & 1.856  & 2.397 &  3.186  &  2.555 \\
        & \text{BC, LQ, K=5}                      & 0.777 &  1.016  &   0.825 & 1.033 &  1.305  & 1.088  & 1.635 &  2.284 &   1.765 & 2.243 &  2.966 &  2.388 \\
        & \text{DIM, LQ, K=1}                     & 0.754 & 0.954 &  0.794 & 1.516 &  1.885  &  1.590  & 1.511 & 2.023  & 1.613  & 3.472 &  4.411 & 3.660 \\
        % \text{DIM, LQ, K=5}         & \bf{0.729} &   0.921 &  \bf{0.768} & 1.422 & 1.757  &  1.489 & \bf{1.498} & 2.006  & \bf{1.600}  & 3.253 & 4.099  &3.423 \\
        \bottomrule
    \end{tabular}
}
\end{table}





\begin{table}[p]
    \centering
    \caption{Uncertainty and Robustness Performance of the two RIP variants. The top performer between the two variants for each metric and dataset split is \textbf{bolded}. Error metrics for computing R-AUC and F1-AUC is \textbf{weightedADE}. See \cref{subsection:sdc_baseline_results} for setup details.}
    \label{table:sdc_uncertainty}
\vspace{0.1in}
\resizebox{1\textwidth}{!}{
    \begin{tabular}{cc|ccc|ccc|ccc|ccc|c}
        \toprule
         \multirow{2}*{Dataset} &  \multirow{2}*{Model} & \multicolumn{3}{c|}{\text{R-AUC}$\downarrow$} & \multicolumn{3}{c|}{\text{F1-AUC} $\uparrow$} & \multicolumn{3}{c|}{\text{F1@}$95$\% $\uparrow$} & \multirow{2}*{ROC-AUC (\%) $\uparrow$} \\
         & & In & Shifted & Full & In & Shifted & Full & In & Shifted & Full &  \\
        \midrule
        \multirow{3}*{Dev} & \text{(BC, LQ, K=1)} & 0.329 & 0.309 & 0.326  & 0.671 & 0.685  & 0.673 & 0.837 & 0.866 &  0.841 &\\
        & \text{BC, LQ, K=5} & 0.529 & 0.488 & 0.525 & 0.552 & 0.607 & 0.558 & 0.801 & 0.835  & 0.805 & \\
        & \text{DIM, LQ, K=1} & 0.497 & 0.455 & 0.492 & 0.623 & 0.647  & 0.626 & 0.797 & 0.862& 0.805 &\\
        % \text{DIM, LQ, K=5} & 0.488 & \bf{0.424} & \bf{0.480} & \bf{0.615} & \bf{0.648} & \bf{0.619} & 0.786 & \bf{0.856} & 0.795 & \\
        \midrule
        \multirow{3}*{Eval} & \text{(BC, LQ, K=1)} & 0.337 & 0.428 & 0.354 & 0.671 & 0.677 & 0.672 & 0.832 &  0.795&  0.825 & \\
        & \text{BC, LQ, K=5} & 0.533 & 0.665 & 0.556& 0.552 & 0.533 & 0.549 & 0.797 &  0.765  & 0.791 & \\
        & \text{DIM, LQ, K=1} & 0.511 & 0.627 & 0.533 & 0.620 & 0.624 & 0.621 & 0.791 & 0.772 & 0.787 & \\
        % \text{DIM, LQ, K=5} & 0.501 & 0.601 & \bf{0.520}  & 0.612 & 0.620 & \bf{0.613}& 0.781 & 0.766 & 0.778  & \\
        \bottomrule
    \end{tabular}
}
\end{table}

\FloatBarrier

\begin{figure}[htbp!]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/SDC - Ret - full_dev.pdf}
         \caption{Joint \texttt{dev} weightedADE retention.}
         \label{fig:sdc_ret_dev}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/SDC - Ret - full_eval.pdf}
         \caption{Joint \texttt{eval} weightedADE retention.}
         \label{fig:sdc_ret_dev}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/SDC - FBeta - full_dev.pdf}
         \caption{Joint \texttt{dev} F1-weightedADE retention.}
         \label{fig:sdc_fbeta_eval}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/SDC - FBeta - full_eval.pdf}
         \caption{Joint \texttt{eval} F1-weightedADE retention.}
         \label{fig:sdc_fbeta_eval}
     \end{subfigure} 
        \caption{weightedADE and F1-weightedADE retention curves on the joint (i.e., containing both the in-distribution and distributionally shifted datapoints) \texttt{dev} (left column) and \texttt{eval} (right column) partitions of the Motion Prediction dataset.
        Top row: retention on weightedADE. Bottom row: retention on F1-weightedADE.
        We vary the backbone model and number of ensemble members, fix the ``Model Averaging'' aggregation strategy for the per-trajectory aggregation operator $\oplus_{\text{plan}}$ and the per--prediction request aggregation operator $\oplus_{\text{pred-req}}$, and otherwise use the standard RIP settings enumerated in \cref{subsection:sdc_baseline_results}.}
        \label{fig:sdc_retention}
\end{figure}

% \begin{figure}[htbp!]
%      \centering
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SDC - weightedADE Ret - DIM__all__dev.pdf}
%          \caption{DIM: joint \texttt{dev} weightedADE retention.}
%          \label{fig:sdc_dim_dev}
%      \end{subfigure}
%      %\hfill
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SDC - weightedADE Ret - BC__all__dev.pdf}
%          \caption{BC: joint \texttt{dev} weightedADE retention.}
%          \label{fig:sdc_bc_dev}
%      \end{subfigure}
%      \\
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SDC - weightedADE Ret - DIM__all__eval.pdf}
%          \caption{DIM: joint \texttt{eval} weightedADE retention.}
%          \label{fig:sdc_dim_eval}
%      \end{subfigure}
%      %\hfill
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SDC - weightedADE Ret - BC__all__eval.pdf}
%          \caption{BC: joint \texttt{eval} weightedADE retention.}
%          \label{fig:sdc_bc_eval}
%      \end{subfigure} 
%         \caption{weightedADE retention curves on the joint (i.e., containing both the in-distribution and distributionally shifted datapoints) \texttt{dev} (top row) and \texttt{eval} (bottom row) partitions of the Motion Prediction dataset.
%         Left column: results using Deep Imitative Model (DIM) \cite{rhinehart2018deep} ensemble members.
%         Right column: using behavioral cloning (BC) \cite{codevilla2018end} ensemble members.
%         Other than varying the backbone model, we use the standard RIP settings enumerated in \cref{subsection:sdc_baseline_results}.}
%         \label{fig:sdc_retention}
% \end{figure}

% \begin{figure}[htbp!]
%      \centering
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SDC - fbeta weightedADE - DIM__all__dev.pdf}
%          \caption{DIM: joint \texttt{dev} F1-weightedADE retention.}
%          \label{fig:sdc_dim_dev_fbeta}
%      \end{subfigure}
%      %\hfill
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SDC - fbeta weightedADE - BC__all__dev.pdf}
%          \caption{BC: joint \texttt{dev} F1-weightedADE retention.}
%          \label{fig:sdc_bc_dev_fbeta}
%      \end{subfigure}
%      \\
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SDC - fbeta weightedADE - DIM__all__eval.pdf}
%          \caption{DIM: joint \texttt{eval} F1-weightedADE retention.}
%          \label{fig:sdc_dim_eval_fbeta}
%      \end{subfigure}
%      %\hfill
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/SDC - fbeta weightedADE - BC__all__eval.pdf}
%          \caption{BC: joint \texttt{eval} F1-weightedADE retention.}
%          \label{fig:sdc_bc_eval_fbeta}
%      \end{subfigure} 
%         \caption{F1-weightedADE retention curves on the joint (i.e., containing both the in-distribution and distributionally shifted datapoints) \texttt{dev} (top row) and \texttt{eval} (bottom row) partitions of the Motion Prediction dataset.
%         Left column: results using Deep Imitative Model \cite{rhinehart2018deep} (DIM) ensemble members.
%         Right column: using behavioral cloning (BC) \cite{codevilla2018end} ensemble members.
%         Other than varying the backbone model, we use the standard RIP settings enumerated in \cref{subsection:sdc_baseline_results}.}
%         \label{fig:sdc_retention_fbeta}
% \end{figure}

\textbf{Retention Results.} 
See \cref{fig:sdc_retention} for weightedADE and F1-weightedADE retention curves across the two RIP variants and the joint (i.e., containing both the in-distribution and distributionally shifted datapoints) \texttt{dev} and \texttt{eval} partitions.
Based on the results shown in \ref{table:sdc_performance}, we find that BC with Model Averaging aggregation achieves the best AUC 
The RIP (DIM) ensemble appears to have significantly higher quality in its per--prediction request uncertainty estimates than RIP (BC). 
For example, on both the joint \texttt{dev} and \texttt{eval} partitions, RIP (BC) has a better weightedADE score at retention fraction 1 (i.e., on all datapoints in the partition), and has a better AUC for its Random and Optimal baselines, which indicates that if uncertainty estimates are of equal quality between the two variants, then RIP (BC) \emph{should perform better}. 
Despite this, the RIP (DIM) AUC-weightedADE is better than those obtained with the BC backbone on both the joint \texttt{dev} and joint \texttt{eval} partitions.
We see that retention using DIM uncertainty scores on both the weightedADE and F1-weightedADE metrics consistently outperforms the Random baseline, unlike the BC uncertainty scores. 
This provides strong evidence that DIM offers better uncertainty quantification than BC on the Vehicle Motion Prediction task.

\FloatBarrier












% \section{SDC Appendix}

% {\color{blue}(Organize in overall appendix)}

% \subsection{Confidence-Aware Metrics}

% \textbf{Normalizing Per-trajectory Confidence Scores.} Note that for RIP, the confidence scores are \emph{meaningful for comparisons across scenes}, i.e., for different prediction request inputs $\bm{x}_i$ and $\bm{x}_j$, we have $c_{d_i} > c_{d_j}$ with $d_i \in \{1, \dots D_i\}, d_j \in \{1, \dots D_j\}$ if the model is more confident about the prediction $d_i$ on input $\bm{x}_i$ than the prediction $d_j$ on input $\bm{x}_j$.
% Importantly, this means that the confidence scores are not (yet) normalized within a particular scene: $\sum_{d_i = 1}^{D_i} c_{d_i} \neq 1, i \in \{i, \dots M\}$ in general. 
% In our case, this is required so that our per--prediction request confidence scores, which are computed via an aggregation over per-trajectory confidence scores, are meaningful. 
% On the other hand, if competitors produce their per--prediction request confidence scores through another manner, their per-trajectory confidence scores may be normalized.
% In all cases, prior to computing the weightedADE and weightedFDE, we apply a \texttt{softmax} over the per-trajectory confidence scores to obtain a normalized distribution.
